The centripetal pull of climate: Evidence from European Parliament elections (1989-2019)

This paper examines the impact of temperature shocks on European Parliament elections. We combine high-resolution climate data with results from parliamentary elections between 1989 and 2019, aggregated at the NUTS-2 regional level. Exploiting exogenous variation in unusually warm and hot days during the months preceding elections, we identify the effect of short-run temperature shocks on voting behaviour. We find that temperature shocks reduce ideological polarisation and increase vote concentration, as voters consolidate around larger, more moderate parties. This aggregated pattern is explained by a gain in support of liberal and, to a lesser extent, social democratic parties, while right-wing parties lose vote share. Consistent with a salience mechanism, complementary analysis of party manifestos shows greater emphasis on climate-related issues in warmer pre-electoral contexts. Overall, our findings indicate that climate shocks can shift party systems toward the centre and weaken political extremes.

==> Table_baselineHHIturnoutBINSyearlybf.tex <==
L1: -30<T<-25       &      -2.206         &      -0.871         &     -26.854         &     -18.710         \\
                    &     (3.245)         &     (3.267)         &    (22.276)         &    (23.021)         \\
L1: -25<T<-20       &       2.437         &       2.978         &      18.850         &      34.956\sym{**} \\
                    &     (1.952)         &     (2.497)         &    (16.280)         &    (13.767)         \\
L1: -20<T<-15       &      -0.760         &       1.160         &      10.831         &      10.846         \\
                    &     (0.972)         &     (1.010)         &    (10.005)         &    (10.172)         \\
L1: -15<T<-10       &      -0.163         &       0.993\sym{**} &      16.274\sym{*}  &       2.661         \\
                    &     (0.424)         &     (0.443)         &     (8.395)         &     (8.283)         \\
L1: -10<T<-5        &       0.157         &       0.488\sym{**} &       0.893         &       4.291         \\
                    &     (0.176)         &     (0.239)         &     (3.089)         &     (3.485)         \\
L1: -5<T<0          &       0.094         &       0.243\sym{***}&       4.494\sym{*}  &       2.852         \\
                    &     (0.076)         &     (0.082)         &     (2.685)         &     (2.028)         \\
L1: 0<T<5           &       0.000         &       0.000         &       0.000         &       0.000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         \\
L1: 5<T<10          &       0.266\sym{***}&       0.051         &      -4.247\sym{**} &      -2.334\sym{*}  \\
                    &     (0.086)         &     (0.054)         &     (1.748)         &     (1.358)         \\
L1: 10<T<15         &       0.314\sym{**} &       0.056         &      -6.315\sym{**} &      -4.261\sym{*}  \\
                    &     (0.126)         &     (0.088)         &     (2.791)         &     (2.248)         \\
L1: 15<T<20         &       0.254\sym{*}  &       0.041         &      -6.007\sym{*}  &      -4.119         \\
                    &     (0.135)         &     (0.095)         &     (3.247)         &     (2.879)         \\
L1: 20<T<25         &       0.199         &       0.111         &     -10.574\sym{**} &      -7.382\sym{**} \\
                    &     (0.153)         &     (0.087)         &     (4.155)         &     (3.610)         \\
L1: 25<T<30         &       0.164         &       0.081         &      -5.989         &      -4.432         \\
                    &     (0.196)         &     (0.124)         &     (5.030)         &     (4.626)         \\
L1: 30<T            &      -0.172         &       0.151         &       1.302         &      -2.305         \\
                    &     (0.773)         &     (0.442)         &     (9.988)         &     (9.067)         \\
R-sq                &       0.981         &       0.973         &       0.901         &       0.917         \\
Observations        &        1055         &        1215         &        1215         &        1215         \\


==> Table_baselineHHIturnoutBINSyearlybfTwmax.tex <==
-15<T<-10           &      0.2778         &      1.1396\sym{***}&     -0.3576         \\
                    &    (0.4421)         &    (0.3913)         &    (5.7721)         \\
-10<T<-5            &     -0.2116         &      0.6744         &      0.9277         \\
                    &    (0.2896)         &    (0.5068)         &    (3.6309)         \\
-5<T<0              &     -0.1300         &      0.3601\sym{**} &      2.1869         \\
                    &    (0.1253)         &    (0.1580)         &    (2.4187)         \\
0<T<5               &     -0.1454\sym{**} &      0.1102\sym{**} &      2.5755         \\
                    &    (0.0575)         &    (0.0534)         &    (1.8479)         \\
5<T<10              &      0.0000         &      0.0000         &      0.0000         \\
                    &         (.)         &         (.)         &         (.)         \\
10<T<15             &      0.1309\sym{*}  &      0.0600         &     -5.7151\sym{***}\\
                    &    (0.0761)         &    (0.0541)         &    (1.8376)         \\
15<T<20             &      0.2230\sym{**} &      0.2026\sym{***}&    -10.1606\sym{***}\\
                    &    (0.0923)         &    (0.0705)         &    (2.7269)         \\
20<T<25             &      0.1765\sym{*}  &      0.2366\sym{***}&    -11.9775\sym{***}\\
                    &    (0.0961)         &    (0.0749)         &    (2.9858)         \\
25<T<30             &      0.1978\sym{*}  &      0.3427\sym{***}&    -14.8454\sym{***}\\
                    &    (0.1132)         &    (0.0815)         &    (3.5528)         \\
30<T<35             &      0.1622         &      0.4099\sym{***}&    -15.0172\sym{***}\\
                    &    (0.1424)         &    (0.0910)         &    (3.8996)         \\
35<T                &     -0.5403         &      0.4278\sym{*}  &     -8.9018\sym{*}  \\
                    &    (0.5628)         &    (0.2529)         &    (4.7013)         \\
R-sq                &       0.979         &       0.969         &       0.912         \\
Observations        &        1283         &        1483         &        1483         \\


==> Table_baselineelectoutomes6mlybf.tex <==
Sum of all temperature coeff.&      -0.003         &       0.008**         &      -0.002         &      -0.006         &       0.003         &      -0.002         &      -0.001         &       0.006**         \\
                    &     (0.003)         &     (0.003)         &     (0.005)         &     (0.004)         &     (0.005)         &     (0.007)         &     (0.004)         &     (0.003)         \\
R-sq                &       0.985         &       0.968         &       0.960         &       0.934         &       0.935         &       0.970         &       0.921         &       0.948         \\
Observations        &        1471         &        1471         &        1471         &        1471         &        1471         &        1471         &        1471         &        1471         \\


==> Table_baselinepolHHIturnoutmonthlybf.tex <==
Sum of all temperature coeff.&      -0.007**         &       0.003         &       0.146         &      -0.334***         \\
                    &     (0.004)         &     (0.005)         &     (0.093)         &     (0.120)         \\
R-sq                &       0.970         &       0.971         &       0.909         &       0.922         \\
Observations        &        1471         &        1471         &        1471         &        1471         \\


==> Table_tempbinsSHLIBSOCRIGhightlowemp8090.tex <==
-15<T<-10           &                     &      -0.404         &                     &       0.402         &                     &      -0.426         \\
                    &                     &     (0.423)         &                     &     (0.632)         &                     &     (0.479)         \\
-10<T<-5            &                     &      -0.323         &                     &       0.015         &                     &       0.078         \\
                    &                     &     (0.232)         &                     &     (0.419)         &                     &     (0.263)         \\
-5<T<0              &      -0.323         &      -0.224         &      -0.442         &       0.117         &      -0.196         &      -0.013         \\
                    &     (0.358)         &     (0.173)         &     (0.334)         &     (0.240)         &     (0.173)         &     (0.202)         \\
0<T<5               &      -0.056         &      -0.221\sym{**} &      -0.391\sym{**} &       0.055         &       0.400         &       0.154         \\
                    &     (0.107)         &     (0.093)         &     (0.170)         &     (0.132)         &     (0.278)         &     (0.137)         \\
5<T<10              &       0.000         &       0.000         &       0.000         &       0.000         &       0.000         &       0.000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         &         (.)         \\
10<T<15             &       0.161\sym{*}  &       0.077         &       0.120         &       0.119         &      -0.263\sym{*}  &      -0.272\sym{*}  \\
                    &     (0.092)         &     (0.089)         &     (0.115)         &     (0.166)         &     (0.152)         &     (0.155)         \\
15<T<20             &       0.331\sym{***}&       0.124         &       0.192         &       0.295         &      -0.376\sym{**} &      -0.389\sym{*}  \\
                    &     (0.112)         &     (0.098)         &     (0.129)         &     (0.215)         &     (0.167)         &     (0.220)         \\
20<T<25             &       0.424\sym{**} &       0.097         &       0.403\sym{**} &       0.306         &      -0.248         &      -0.342         \\
                    &     (0.175)         &     (0.126)         &     (0.178)         &     (0.269)         &     (0.179)         &     (0.284)         \\
25<T<30             &       0.448\sym{**} &       0.191         &       0.608\sym{**} &       0.503         &      -0.397\sym{**} &      -0.201         \\
                    &     (0.172)         &     (0.156)         &     (0.305)         &     (0.337)         &     (0.165)         &     (0.374)         \\
30<T<35             &       0.502\sym{***}&       0.675\sym{*}  &       0.713\sym{*}  &      -0.409         &      -0.537\sym{**} &      -0.027         \\
                    &     (0.190)         &     (0.383)         &     (0.365)         &     (0.541)         &     (0.220)         &     (0.453)         \\
35<T                &       0.590\sym{*}  &                     &       0.893         &                     &      -0.137         &                     \\
                    &     (0.313)         &                     &     (1.056)         &                     &     (0.328)         &                     \\
R-sq                &       0.956         &       0.967         &       0.951         &       0.924         &       0.922         &       0.957         \\
Observations        &         733         &         718         &         733         &         718         &         733         &         718         \\


==> Table_tempbinsmanifestosyear.tex <==
(-15<T<-10)         &       2.137         &       2.145         &       2.126         \\
                    &     (1.336)         &     (1.344)         &     (1.337)         \\
(-25<T<-20)$\times$ Lib party&      -5.168\sym{*}  &      -5.110\sym{*}  &      -5.104\sym{*}  \\
                    &     (2.209)         &     (2.219)         &     (2.209)         \\
(-10<T<-5)          &      -0.325         &      -0.330         &      -0.328         \\
                    &     (0.193)         &     (0.194)         &     (0.192)         \\
(-10<T<-5)$\times$ Lib party&       0.453         &       0.418         &       0.412         \\
                    &     (0.244)         &     (0.233)         &     (0.228)         \\
(-5<T<0)            &       0.079         &       0.083         &       0.089         \\
                    &     (0.182)         &     (0.182)         &     (0.181)         \\
(-5<T<0)$\times$ Lib party&       0.480\sym{***}&       0.459\sym{***}&       0.453\sym{***}\\
                    &     (0.101)         &     (0.094)         &     (0.092)         \\
(0<T<5)             &      -0.126\sym{**} &      -0.124\sym{**} &      -0.125\sym{**} \\
                    &     (0.045)         &     (0.044)         &     (0.043)         \\
(0<T<5)$\times$ Lib party&      -0.048\sym{**} &      -0.046\sym{*}  &      -0.046\sym{*}  \\
                    &     (0.019)         &     (0.020)         &     (0.021)         \\
(5<T<10)            &       0.000         &       0.000         &       0.000         \\
                    &         (.)         &         (.)         &         (.)         \\
(10<T<15)           &       0.289         &       0.284         &       0.288         \\
                    &     (0.207)         &     (0.209)         &     (0.208)         \\
(10<T<15)$\times$ Lib party&       0.279\sym{***}&       0.262\sym{***}&       0.257\sym{***}\\
                    &     (0.073)         &     (0.066)         &     (0.064)         \\
(15<T<20)           &       0.262         &       0.256         &       0.257         \\
                    &     (0.150)         &     (0.153)         &     (0.152)         \\
(15<T<20)$\times$ Lib party&       0.055         &       0.048         &       0.047         \\
                    &     (0.044)         &     (0.046)         &     (0.046)         \\
(20<T<25)           &       0.160         &       0.148         &       0.148         \\
                    &     (0.116)         &     (0.118)         &     (0.118)         \\
(20<T<25)$\times$ Lib party&       0.579\sym{***}&       0.551\sym{***}&       0.544\sym{***}\\
                    &     (0.163)         &     (0.154)         &     (0.151)         \\
(25<T<30)           &       0.109         &       0.098         &       0.099         \\
                    &     (0.074)         &     (0.075)         &     (0.075)         \\
(25<T<30)$\times$ Lib party&       0.091         &       0.064         &       0.057         \\
                    &     (0.064)         &     (0.061)         &     (0.060)         \\
(30<T<35)           &      -0.153\sym{***}&      -0.162\sym{***}&      -0.164\sym{***}\\
                    &     (0.030)         &     (0.032)         &     (0.033)         \\
(30<T<35)$\times$ Lib party&       1.170\sym{**} &       1.255\sym{**} &       1.284\sym{**} \\
                    &     (0.463)         &     (0.445)         &     (0.436)         \\
R-sq                &       0.649         &       0.641         &       0.637         \\
Observations        &          99         &          99         &          99         \\


==> Table_tempbinsshlibpolarl1hightlowemp8090.tex <==
-15<T<-10           &                     &                     &      -2.176         &      -0.404         \\
                    &                     &                     &     (6.290)         &     (0.423)         \\
-10<T<-5            &                     &                     &       1.593         &      -0.323         \\
                    &                     &                     &     (3.845)         &     (0.232)         \\
-5<T<0              &       4.034         &      -0.323         &       1.062         &      -0.224         \\
                    &    (10.352)         &     (0.358)         &     (2.727)         &     (0.173)         \\
0<T<5               &       2.392         &      -0.056         &       2.346         &      -0.221\sym{**} \\
                    &     (4.369)         &     (0.107)         &     (2.012)         &     (0.093)         \\
5<T<10              &       0.000         &       0.000         &       0.000         &       0.000         \\
                    &         (.)         &         (.)         &         (.)         &         (.)         \\
10<T<15             &      -7.394\sym{***}&       0.161\sym{*}  &      -4.619\sym{*}  &       0.077         \\
                    &     (2.704)         &     (0.092)         &     (2.786)         &     (0.089)         \\
15<T<20             &     -11.837\sym{***}&       0.331\sym{***}&      -8.345\sym{**} &       0.124         \\
                    &     (4.324)         &     (0.112)         &     (3.977)         &     (0.098)         \\
20<T<25             &     -14.152\sym{***}&       0.424\sym{**} &      -9.551\sym{**} &       0.097         \\
                    &     (4.905)         &     (0.175)         &     (4.619)         &     (0.126)         \\
25<T<30             &     -17.687\sym{***}&       0.448\sym{**} &     -12.228\sym{**} &       0.191         \\
                    &     (5.149)         &     (0.172)         &     (5.893)         &     (0.156)         \\
30<T<35             &     -19.062\sym{***}&       0.502\sym{***}&      -3.216         &       0.675\sym{*}  \\
                    &     (5.412)         &     (0.190)         &     (5.288)         &     (0.383)         \\
35<T                &     -15.161\sym{***}&       0.590\sym{*}  &                     &                     \\
                    &     (5.122)         &     (0.313)         &                     &                     \\
R-sq                &       0.908         &       0.956         &       0.924         &       0.967         \\
Observations        &         733         &         733         &         718         &         718         \\

